Automated Reporting of GUI Design Violations for Mobile Apps

The inception of a mobile app often takes form of a mock-up of the Graphical User Interface (GUI), represented as a static image delineating the proper layout and style of GUI widgets that satisfy requirements. Following this initial mock-up, the design artifacts are then handed off to developers whose goal is to accurately implement these GUIs and the desired functionality in code. Given the sizable abstraction gap between mock-ups and code, developers often introduce mistakes related to the GUI that can negatively impact an app's success in highly competitive marketplaces. Moreover, such mistakes are common in the evolutionary context of rapidly changing apps. This leads to the time-consuming and laborious task of design teams verifying that each screen of an app was implemented according to intended design specifications. This paper introduces a novel, automated approach for verifying whether the GUI of a mobile app was implemented according to its intended design. Our approach resolves GUI-related information from both implemented apps and mock-ups and uses computer vision techniques to identify common errors in the implementations of mobile GUIs. We implemented this approach for Android in a tool called GVT and carried out both a controlled empirical evaluation with open-source apps as well as an industrial evaluation with designers and developers from Huawei. The results show that GVT solves an important, difficult, and highly practical problem with remarkable efficiency and accuracy and is both useful and scalable from the point of view of industrial designers and developers. The tool is currently used by over one-thousand industrial designers and developers at Huawei to improve the quality of their mobile apps.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	


\newcommand\KEVIN[1]{{\color{blue} \nb{KEVIN}{#1}}}
\newcommand\BOYANG[1]{{\color{blue}\nb{BOYANG}{#1}}}
\newcommand\DENYS[1]{{\color{blue}\nb{DENYS}{#1}}}
\newcommand\DAN[1]{{\color{blue}\nb{DAN}{#1}}}
\newcommand\CARLOS[1]{{\color{blue}\nb{CARLOS}{#1}}}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> prototype.tex <==
% !TEX root = main.tex

%-----------------------------------------------
\subsection{Huawei Prototype Progression}
\label{subsec:prototype}

	The development cycle will result in two major prototype releases for Huawei: \textit{Prototype v1} and \textit{Prototype v2}.  The expected inputs, outputs, and requirements for each of these prototypes are listed below:
	\\
	
\begin{figure*}[tb]
\centering
\vspace{-0.7cm}
\includegraphics[width=\linewidth]{img/GUI-Verification-Architecture-Desktop.pdf}
\vspace{-0.5cm}
\caption{Architecture Option 1: Desktop Application}
\label{fig:desktop-design}
\end{figure*}

\begin{figure*}[tb]
\centering
\includegraphics[width=\linewidth]{img/GUI-Verification-Architecture-Phone.pdf}
\vspace{-0.5cm}
\caption{Architecture Option 2: Android Application}
\label{fig:phone-design}
\vspace{-0.3cm}
\end{figure*}
	

	
	\textit{\textbf{Prototype v1:}} 
	
	\begin{itemize}
	
	\item{\textit{Inputs:} This version of the tool takes as input two \textit{design mock-ups} (e.g. \texttt{Marketch} files), one \textit{annotated} and one \textit{non-annotated}; It will also take an \texttt{xml ui-dump} obtained from the \texttt{uiautomator} tool and screenshot from an Android application corresponding to the design screen.}
	
	\item{\textit{Outputs:} The output will be a text file with accurate natural language descriptions of violations and a set of augmented screenshots that further delineate detected design errors.}
	
	\item{\textit{Requirements:} 1) Should parse the non-annotated Marketch file to build a GUI-hierarchy for the design mockup;  2) Should parse the Android \texttt{ui-dump} xml file to build a GUI-hierarchy for the app implementation; 3) Should modify the design mock-up GUI-hierarchy by detecting and dividing parent containers based on line splitters, as described in Section \ref{subsubsec:transformations}; 4) Should modify the GUI-hierarchy of the app implementation by applying the transformation heuristics described in Section \ref{subsubsec:transformations}; 5) Should perform recursive tree resolution as described in Section \ref{subsubsec:transformations} 6) Should perform component matching as described in Section \ref{subsubsec:comp-matching}; 7) Should detect and report the following types of violations: (i) Layout Violations, (ii) Missing Component Violations, (iii) Extraneous Component Violations; 8) Should output a textual description of each design violation detected including the type of violation, identifying information about the components involved in the violation, and a brief delineation of the reason for the violation.  9) Should achieve a recall of at least 60\% for the three violation types indicated in Requirement 7 in the context of the study described in Section \ref{sec:study}; 10) Should achieve a precision of at least 60\% for the three types of violations listed in Requirement 7 in the context of the study described in Section \ref{sec:study}.}
	
	\end{itemize}
	
	\textit{\textbf{Prototype v2:}} 
	
	\begin{itemize}
	
	\item{\textit{Inputs:} This version of the tool takes as input two \textit{design mock-ups} (e.g. \texttt{Marketch} files), one \textit{annotated} and one \textit{non-annotated}; It will also take a .apk file from an Android application corresponding to the design screen. The .apk file must be installed on a target device.}
	
	\item{\textit{Outputs:} The output will consist of an html report containing natural language descriptions of design violations and corresponding augmented screenshots illustrating the components that were involved in the violations.}
	
	\item{\textit{Requirements:} This prototype will implement Requirements 1-7 listed above as well as the following new requirements: 1) Should allow the developer to semi automatically capture GUI information from a running Android app on either a physical device or emulator, either by connecting the device to a PC, or utilizing an companion Android app with screen overlay interface to capture particular GUI screens;  2) Should utilize a user-interface instantiated either in a Java-based Desktop Application, or Android Application.  3) Should allow a user to specify matches between Marketch Files and App implementation screenshots to allow for intended analysis.  4) Should generate html based reports viewable in the GUI of the \GuiFitsp tool. 5) Should further detect and report the following violation types: (i) Component Size Violations, (ii) Text Mismatches;  6) Should achieve a recall of at least 70\% for the five specified violation types in the context of the study described in Section \ref{sec:study}; 7) Should achieve a precision of at least 70\% for the five specified violation types in the context of the study described in Section \ref{sec:study}.}
	
	\end{itemize}
	
%-----------------------------------------------
\subsection{Options for Tool Architecture}

	There are two major options for implementing the architecture of the prototype \GuiFitsp tool.  The first is a standalone Java Desktop application that would require a connection to an Android device to collect GUI Information from a running application. The second is an implementation of the \GuiFitsp approach self-contained within an Android application.  A brief description of the workflow and positives and negatives of each architecture implementation are outlined below.
	
%-----------------------------------------------
\subsubsection{Desktop Application Implementation}

In this option \GuiFitsp would function as Java Desktop PC application as specified in Figure \ref{fig:desktop-design}.  The Marketch files would be selected in a File browsing interface of the GUI of the Desktop PC app and the information from the Android app would be uploaded either via a Collector App or by connecting an Android device or emulator to a PC.  In the Collector App, a user would be able to use either an emulator or physical device connected to the Desktop PC and launch the app they would like to collect GUIs for, and then press a screen overlay button to automatically send the GUI to the Desktop Application.  Alternatively, we could keep the button to collect the GUI information on the Desktop App.  If the button were instead to exist only in the Desktop PC app, then there would be no need for a separate Android app.  Instead, the user would simply launch the app they would like to collect the screen information from, connect the device to the PC, and press the button in the GUI to collect the GUI information for the current static screen in the Android app.  Next the developer would select which Marketch files correspond to the proper Android app screens, and further select which pairs of design and implementation screens to run the analysis on.  The output would be an html report of all screen analysis pairs.

\textbf{Pros:}

\begin{itemize}

\item{Able to upload screen information for multiple types of Android devices to have reports aggregated in one place.}
\item{Java app should run on any OS or type of Desktop PC (as long as Java is installed).}
\item{Easy to upload Marketch Files on the PC.}

\end{itemize}

\textbf{Cons:}

\begin{itemize}

\item{Effort required to connect device to PC or start emulator to collect Android data.}
\item{Potentially two different pieces of code to develop and maintain.}
\item{Might require installation of the Android SDK on the host machine.}

\end{itemize}

%-----------------------------------------------
\subsubsection{Android Application Implementation}

In this option, \GuiFitsp would be self-contained within an Android application and follow the workflow outlined in Figure \ref{fig:phone-design}.  The workflow would be as follows: First, a user would launch the GVT .apk in either a physical device or emulator.  Then they would connect this device to their Desktop PC and upload the Marketch files to a pre-designated folder on the Android device.  Then they would open the app they would like to analyze on the Android device, and press a button appearing as a screen overlay to automatically capture the GUI information.  They would then select the proper Marketch-screenshot pairs to run the violation detection analysis on, and specify how many screen pairs should be analyzed.  Then the app would perform the violation analysis and display results on the screen of the phone.

\textbf{Pros:}

\begin{itemize}

\item{Self-contained app, entire process can be performed on smartphone or tablet.}
\item{Easy to acquire Android information on the device.}

\end{itemize}

\textbf{Cons:}

\begin{itemize}

\item{Effort required to upload Marketch files to device}
\item{Only reports for the single type of Android device the app is installed on can be created.  The app will have to be installed on multiple devices and all the reports would reside on the individual devices unless sent to a centralized place.}
\item{Smartphone or tablet screen may not be as optimal for viewing reports.}
\item{Computational intensity of the tool may cause it to be slower on the phone (We would need to test)}
\item{Would probably require more development time.}

\end{itemize}

%-----------------------------------------------
\subsection{Specified Protoype Limitations}

	The \GuiFitsp tool will implemented as a \textit{prototype} for internal use in Huawei, and will not resemble a production quality tool.  \textit{\textbf{Prototype v2}} will be relatively full-featured as described by the requirements stipulated in Section \ref{subsec:prototype}.  However, there are some noteworthy limitations that the UI/UX team should be made aware of.  The following limitations apply to both versions of the prototypes.  
	
	First, the tool will not be able to analyze design mock-up screens that extend beyond the bounds of a typical device screen.  This means instances of UI designs where lists that extend vertically below the typical bounds of a device screen will not be properly analyzed.  Second, the prototypes will not be able to analyze screens corresponding to design mock-ups that include onscreen soft-keyboards.  This is an inherent limitation of the \texttt{uiautomator} tool, as it is not able to properly record the keyboard displayed on device screens.  Third, the prototype will only handle the violation types specified in the requirements outlined in Section \ref{subsec:prototype}.  The violation types not considered by the prototypes are classified as technically challenging and would most likely require more research and experimentation to implement properly.  However, there may be an opportunity to implement these in the future as the collaboration continues.  Fourth, The prototypes will not able to detect violations between two screens with a high number of structural differences. That is, the prototypes will expect that the screens represented in the Marketch Files and captured in the app implementation, share a high degree of structural similarity or visually represent the same screen. Fifth, the prototypes will only consider the types of annotations discussed in Section \ref{subsubsec:annotations}, as further types of annotations are too ambiguous for our tool to comprehend.  Finally, there may be further unexpected limitations of the prototype implementations, including crashes or unexpected behavior in corner cases, and lower than expected performance for certain app screens with unexpected GUI structures.

